SuperFusion: Multilevel LiDAR-Camera Fusion for Long-Range HD Map Generation

High-definition (HD) semantic map generation of the environment is an essential component of autonomous driving. Existing methods have achieved good performance in this task by fusing different sensor modalities, such as LiDAR and camera. However, current works are based on raw data or network feature-level fusion and only consider short-range HD map generation, limiting their deployment to realistic autonomous driving applications. In this paper, we focus on the task of building the HD maps in both short ranges, i.e., within 30 m, and also predicting long-range HD maps up to 90 m, which is required by downstream path planning and control tasks to improve the smoothness and safety of autonomous driving. To this end, we propose a novel network named SuperFusion, exploiting the fusion of LiDAR and camera data at multiple levels. We use LiDAR depth to improve image depth estimation and use image features to guide long-range LiDAR feature prediction. We benchmark our SuperFusion on the nuScenes dataset and a self-recorded dataset and show that it outperforms the state-of-the-art baseline methods with large margins on all intervals. Additionally, we apply the generated HD map to a downstream path planning task, demonstrating that the long-range HD maps predicted by our method can lead to better path planning for autonomous vehicles. Our code has been released at https://github.com/haomo-ai/SuperFusion.

==> stachnisslab-math.tex <==
%% Math definitions used at the Stachniss-Lab

% argmax operator
\def\argmax{\mathop{\rm argmax}}

% argmain operator
\def\argmin{\mathop{\rm argmin}}

%% Spaces
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}

% O-Notation
\newcommand{\bigO}[1]{$\mathcal{O}(#1)$}

% absolute value
\newcommand{\abs}[1]{|#1|}

% Norm
\newcommand{\norm}[1]{\lVert#1\lVert}

% 1/2 as math
\newcommand{\half}{\frac{1}{2}}

% sign 
\newcommand{\sign}[0]{{\mbox{sign}}}

% specif matrix dimensions under a matrix
\newcommand{\mdim}[3]{\stackrel[\mbox{\tiny $#2\!\!\times\!\!#3$}]{}{#1}}

% math boldface #1  
\renewcommand{\b}[1]{\mbox{\boldmath$#1$}}

% =\b (for compatability)
\renewcommand{\d}[1]{\b {#1}}

% vector
\renewcommand{\v}[1]{{\b #1}} 

% matrix
\newcommand{\m}[1]{{\mbox{{\sffamily\slshape{#1\/}}}}}

% homogeneous vector
\newcommand{\q}[1]{{{\bf #1}}}

% homogeneous matrix
\newcommand{\mq}[1]{{\mbox{{\sffamily{#1}}}}}

% transpose vector or matrix
\newcommand{\tr}[0]{\sf T}              % transpose without ^  
\newcommand{\trans}[0]{^\tr}            % normal
\newcommand{\transs}[0]{{'}^\tr}        % ‘ trans
\newcommand{\transss}[0]{{''}^\tr}      % ‘‘ trans
\newcommand{\transsss}[0]{{'''}^\tr}    % ’’’ trans
\newcommand{\transi}[0]{^{-\tr}}        % - trans
\newcommand{\transa}[0]{^{*\tr}}        % * trans

%inverse 
\newcommand{\inv}{^{-1}}

% Differential operator d
\newcommand{\diff}[0]{\mbox{d}}

% degree
\newcommand{\degrees}{{\mbox{$^\circ$}}}

% Diag 
\newcommand{\Diag}[0]{{\mbox{Diag}}}

% trace  
\newcommand{\trace}[0]{{\mbox{tr}\,}}

% rank 
\newcommand{\rank}[0]{{\mbox{rank}\,}}

% nullspace 
\newcommand{\nullspace}[0]{{\mbox{null}}}

%atan2 (use with one argument: sin- and cos-part  seperated by , or ;)
\newcommand{\atan}[1]{\mbox{atan2} \, ({#1})}

%acot2 (use with one argument: sin- and cos-part  seperated by , or ;)
\newcommand{\acot}[1]{\mbox{acot2} \, ({#1})}

% specify coordinate system of an element
%#1 = system, #2 = variable
\newcommand{\cs}[2]{\; ^{#1}\!\,{\mbox{#2}}}

% specify coordinate system of matrix from to
% #1 = variable, #2 = from, #3 = to,
\newcommand{\cft}[3]{\; ^{#1}\!\,{\mbox{#2}}_{#3}}

%Rotationmatrix with index and angle: R_i(a)%
\newcommand{\rot}[2]{\m{R}_{#1}(#2)}

%Rotationmatrix transposed with index and angle:  R^T_i(a)%
\newcommand{\rott}[2]{\m{R}\trans_{#1}(#2)}

% Jacobian
\newcommand{\J}{\m J} 


%2 vector%
\newcommand{\zvector}[2]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2}
        \end{array}
       \right] }

%3 vector%
\newcommand{\dvector}[3]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3}
        \end{array}
       \right] }

%4 vector%
\newcommand{\vvector}[4]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}
          \end{array}
       \right] }

%5 vector%
\newcommand{\fvector}[5]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}
          \end{array}
       \right] }

%%6 vector%
\newcommand{\svector}[6]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}
          \end{array}
       \right] }

%%7 vector%
\newcommand{\sivector}[7]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}
          \end{array}
       \right] }

%%8 vector%
\newcommand{\avector}[8]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}\\ {#8}
          \end{array}
       \right] }
       
%%9 vector%
\newcommand{\nvector}[9]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}\\ {#8}\\ {#9}
          \end{array}
       \right] }


%2 vector transposed%
\newcommand{\zvectort}[2]
  {    \left[
            {#1} \; {#2}
       \right] }


%3 vector transposed%
\newcommand{\dvectort}[3]
  {    \left[
            {#1} \; {#2}\; {#3}
       \right] }

%4 vector transposed%
\newcommand{\vvectort}[4]
  {    \left[
            {#1} \; {#2}\; {#3}\; {#4}
       \right] }


%2 x 3 matrix%
\newcommand{\zdmatrix}[6]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} & {#3} \\
            {#4} & {#5} & {#6} 
          \end{array}
       \right] }

%2 x 4 matrix%
\newcommand{\zvmatrix}[8]
  {    \left[
          \begin{array}{cccc}
            {#1} & {#2} & {#3} & {#4}\\
            {#5} & {#6} & {#7} & {#8}
          \end{array}
       \right] }
%4 x 2 matrix%
\newcommand{\vzmatrix}[8]
  {    \left[
          \begin{array}{cc}
            {#1} & {#2} \\ {#3} & {#4}\\
            {#5} & {#6} \\ {#7} & {#8}
          \end{array}
       \right] }

%3 x 2 matrix%
\newcommand{\dzmatrix}[6]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} \\
            {#3} & {#4} \\
            {#5} & {#6}
          \end{array}
       \right] }
%

%2 x 2 matrix%
\newcommand{\zmatrix}[4]
  {    \left[
          \begin{array}{cc}
            {#1} & {#2} \\
            {#3} & {#4}
          \end{array}
       \right] }

%3 x 3 matrix%
\newcommand{\dmatrix}[9]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} & {#3} \\
            {#4} & {#5} & {#6} \\
            {#7} & {#8} & {#9}
          \end{array}
       \right] }

%4 x 4 matrix%
%% not allowed, max 9 parameters!

%Determinant 2x2
\newcommand{\zdet}[4]
  {    \left|
          \begin{array}{cc}
            {#1} & {#2} \\
            {#3} & {#4}
          \end{array}
       \right| }

%Determinant 3x3
\newcommand{\ddet}[9]
  {    \left|
          \begin{array}{ccc}
            {#1} & {#2} & {#3}\\
            {#4} & {#5} & {#6}\\
            {#7} & {#8} & {#9}
          \end{array}
       \right| }


 
% General matrix: #1: #colums, #2: String for elemets
% incl. //
\newcommand{\matr}[2]{%
\left[ \begin{array}{*#1{c} }    #2   \end{array} \right] %
  }

 % General Determinant:  #1: #colums, #2: String for elemets
% incl. //
\newcommand{\dete}[2]{%
\left| \begin{array}{*#1{c}}    #2   \end{array} \right| %
  }

 % Boldface abbrevs
\newcommand{\bA}{\b A}
\newcommand{\bB}{\b B}
\newcommand{\bC}{\b C}
\newcommand{\bD}{\b D}
\newcommand{\bE}{\b E}
\newcommand{\bF}{\b F}
\newcommand{\bG}{\b G}
\newcommand{\bH}{\b H}
\newcommand{\bI}{\b I}
\newcommand{\bJ}{\b J}
\newcommand{\bK}{\b K}
\newcommand{\bL}{\b L}
\newcommand{\bM}{\b M}
\newcommand{\bN}{\b N}
\newcommand{\bO}{\b O}
\newcommand{\bP}{\b P}
\newcommand{\bQ}{\b Q}
\newcommand{\bR}{\b R}
\newcommand{\bS}{\b S}
\newcommand{\bT}{\b T}
\newcommand{\bU}{\b U}
\newcommand{\bV}{\b V}
\newcommand{\bW}{\b W}
\newcommand{\bX}{\b X}
\newcommand{\bY}{\b Y}
\newcommand{\bZ}{\b Z}

\newcommand{\ba}{\b a}
\newcommand{\bb}{\b b}
\newcommand{\bc}{\b c}
\newcommand{\bd}{\b d}
\newcommand{\be}{\b e}
%\newcommand{\bf}{\b f}
\newcommand{\bg}{\b g}
\newcommand{\bh}{\b h}
\newcommand{\bi}{\b i}
\newcommand{\bj}{\b j}
\newcommand{\bk}{\b k}
\newcommand{\bl}{\b l}
\newcommand{\bm}{\b m}
\newcommand{\bn}{\b n}
\newcommand{\bo}{\b o}
\newcommand{\bp}{\b p}
\newcommand{\bq}{\b q}
\newcommand{\br}{\b r}
\newcommand{\bs}{\b s}
\newcommand{\bt}{\b t}
\newcommand{\bu}{\b u}
\newcommand{\bv}{\b v}
\newcommand{\bw}{\b w}
\newcommand{\bx}{\b x}
\newcommand{\by}{\b y}
\newcommand{\bz}{\b z}

\newcommand{\dA}{\b A}
\newcommand{\dB}{\b B}
\newcommand{\dC}{\b C}
\newcommand{\dD}{\b D}
\newcommand{\dF}{\b F}
\newcommand{\dG}{\b G}
\newcommand{\dH}{\b H}
\newcommand{\dI}{\b I}
\newcommand{\dJ}{\b J}
\newcommand{\dK}{\b K}
\newcommand{\dL}{\b L}
\newcommand{\dM}{\b M}
\newcommand{\dN}{\b N}
\newcommand{\dO}{\b O}
\newcommand{\dP}{\b P}
\newcommand{\dQ}{\b Q}
\newcommand{\dR}{\b R}
\newcommand{\dS}{\b S}
\newcommand{\dT}{\b T}
\newcommand{\dU}{\b U}
\newcommand{\dV}{\b V}
\newcommand{\dW}{\b W}
\newcommand{\dX}{\b X}
\newcommand{\dY}{\b Y}
\newcommand{\dZ}{\b Z}

\newcommand{\mA}{\m A}
\newcommand{\mB}{\m B}
\newcommand{\mC}{\m C}
\newcommand{\mD}{\m D}
\newcommand{\mF}{\m F}
\newcommand{\mG}{\m G}
\newcommand{\mH}{\m L}
\newcommand{\mI}{\m I}
\newcommand{\mJ}{\m J}
\newcommand{\mK}{\m K}
\newcommand{\mL}{\m L}
\newcommand{\mM}{\m M}
\newcommand{\mN}{\m N}
\newcommand{\mO}{\m O}
\newcommand{\mP}{\m P}
\newcommand{\mQ}{\m Q}
\newcommand{\mR}{\m R}
\newcommand{\mS}{\m S}
\newcommand{\mT}{\m T}
\newcommand{\mU}{\m U}
\newcommand{\mV}{\m V}
\newcommand{\mW}{\m W}
\newcommand{\mX}{\m X}
\newcommand{\mY}{\m Y}
\newcommand{\mZ}{\m Z}



==> tabs/AP_haomo.tex <==
\begin{table*}[!tb]	
\centering
\addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{5pt}
\caption{Instance detection results on self-recorded dataset. The predefined threshold of Chamfer distance is 1.0 m and threshold of IoU is 0.1 (\eg a prediction is considered as a true positive if and only if the CD is below and the IoU is above the defined thresholds). AP: higher is better.}
\label{tab:ap_haomo}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}}& \multicolumn{2}{c}{\textbf{{\scriptsize Average AP}}}\\

& & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C & 40.9  &28.9   &36.2  & 27.1 & 21.9   & 20.0  & 33.0 & 25.4\\
LSS \cite{philion2020lift} & C & 42.8  & 28.9  & 42.7 & 27.7 & 35.8   & 22.9 & 40.4 &26.5 \\
\hline
PointPillars \cite{lang2019pointpillars} & L & 30.7   & 29.0  & 28.0  & 27.6 &  19.7  & 17.2 &  26.1& 24.6\\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L & 44.9  & 29.2  & 43.0 & 28.1 &  27.1  & 19.9 & 38.3 & 25.7\\
BEVFusion \cite{liang2022bevfusion}& C+L & 42.1 & 34.2  & 40.4 & 31.9 & 33.9   &25.2  & 38.8 & 30.5\\
BEVFusion \cite{liu2022bevfusion}& C+L & 43.0   & 28.8  &42.6  & 27.5 & \textbf{35.9}   &21.4  &40.5  &25.9 \\
SuperFusion (ours) & C+L & \textbf{47.5}  & \textbf{38.0} & \textbf{44.3} & \textbf{36.8}  &35.3  & \textbf{30.0}  & \textbf{42.4} & \textbf{35.0} \\
\hline
\end{tabular}
% }
\normalsize
\end{table*}



==> tabs/CD.tex <==
% \begin{table*}[!tb]	
% \centering
% % \addtolength{\tabcolsep}{0.5pt}
% \renewcommand\arraystretch{1}
% \setlength{\tabcolsep}{3pt}
% \caption{Chamfer distance (m) of semantic map segmentation on nuScenes dataset. CD: lower is better.  }
% \label{tab:cd}
% \footnotesize

% \begin{tabular}{c|c|ccc|ccc|ccc|ccc}
% \hline
% \multirow{2.5}{*}{\textbf{Method}} &
% \multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{3}{c}{\textbf{{\scriptsize Average CD}}} \\

% & & {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }\\

% \hline 
% VPN \cite{Pan_2020} & C & 1.001  &0.749   &0.547    &  1.293& 1.003  & 0.763  & 1.394  &\textbf{0.619}   &0.923 &1.232 & 0.847& 0.738\\
% LSS \cite{philion2020lift} & C & 0.819  &0.612   &0.382    &1.024  & 1.091  &  0.528 &  1.096 & 0.695  & 0.701& 0.967& 0.763&0.515 \\
% \hline
% PointPillars \cite{lang2019pointpillars} & L & 0.759  & 0.599  &0.221    & 0.941 & 0.650  &0.425   &1.249   &0.988   &0.747& 0.841& 0.620& 0.316\\
% \hline 
% HDMapNet \cite{li2021hdmapnet}& C+L & 0.641  &0.602   &0.241    &  0.876& 0.976  &0.461   &1.087   &0.960   & 0.775 & 0.822& 0.743& 0.425\\
% BEVFusion \cite{liang2022bevfusion}& C+L&  0.757 & 0.668  &0.250    & 0.894 & 0.810  &0.444   & 0.951  &2.547   & 0.768 & 0.840& 0.862& 0.397\\
% BEVFusion \cite{liu2022bevfusion}& C+L & 0.600  &0.465   &\textbf{0.194}    & 0.798 & 0.562  &\textbf{0.342}   & 0.923  & 0.735  &\textbf{0.494}& 0.734& 0.510& \textbf{0.300}\\
% SuperFusion (ours) & C+L & \textbf{0.531}  & \textbf{0.421}  &   0.211 & \textbf{0.710} &  \textbf{0.434} &  0.399 & \textbf{0.827}  & 0.750  &0.547 &\textbf{0.659} &\textbf{0.458} & 0.342\\
% \hline
% \end{tabular}

% \normalsize
% \vspace{-0.2cm}
% \end{table*}


\begin{table*}[!tb]	
\centering
% \addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{2pt}
\caption{Chamfer distance (m) of semantic map segmentation on nuScenes dataset. CD: lower is better.  }
\label{tab:cd}
\footnotesize

\begin{tabular}{c|c|ccc|ccc|ccc|ccc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{3}{c}{\textbf{{\scriptsize Average CD}}} \\

& & {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C & 3.212  &  4.521 & 3.279   & 2.970  & 4.734  & 2.814   &  2.998  &  5.000  &  3.622 &  3.066  &    4.729 &     3.217\\
LSS \cite{philion2020lift} & C & 2.123  &  3.168 &  2.043  &  2.376 &  4.908 &  2.426  &  2.409  &  5.000  & 3.033  &  2.290  & 4.223    & 2.454    \\
\hline
PointPillars \cite{lang2019pointpillars} & L & 1.691  & 2.661  &  0.929 & 4.049  & 4.646  &  3.503  &  5.000  &  4.958  & 5.000  & 3.515   & 3.818 & 3.190 \\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L & 1.473  & 2.284  &  0.779  & 2.456  &  4.210 &  1.947  &  2.905  &  5.000  &  3.466 &   2.185 & 3.598 & 1.869 \\
BEVFusion \cite{liang2022bevfusion}& C+L&  1.702 & 2.283  &  1.212  &  2.816 &  4.237 &  2.929  &  3.490  &  5.000  & 4.915  & 2.534   & 3.588 &  2.701 \\
BEVFusion \cite{liu2022bevfusion}& C+L & 1.384  & 2.036  &  0.773  & 2.523  & 3.762  &  2.106  & 3.102 & 5.000 & 3.754  & 2.213   &  3.282& 1.980    \\
SuperFusion (ours) & C+L & \textbf{1.305}  & \textbf{1.503}  &  \textbf{0.542}  & \textbf{1.756} &  \textbf{2.641} & \textbf{1.235}  & \textbf{1.964}  &  \textbf{4.081} & \textbf{2.221}&\textbf{1.642} &\textbf{2.449} &\textbf{1.228} \\
\hline
\end{tabular}

\normalsize
\vspace{-0.2cm}
\end{table*}

==> tabs/CD_haomo.tex <==
\begin{table*}[!tb]	
\centering
\addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{5pt}
\caption{Chamfer distance (m) of semantic map segmentation on self-recorded dataset. CD: lower is better. }
\label{tab:cd_haomo}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{2}{c}{\textbf{{\scriptsize Average CD}}} \\

& & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C & 1.058   & 3.280   & 1.298  & 3.980  & 2.657&  4.501 & 1.638  & 3.915 \\
LSS \cite{philion2020lift} & C&  1.067  & 3.579   & 1.048  & 4.074  &  2.412   & 5.000  &  1.244 & 4.111 \\
\hline
PointPillars \cite{lang2019pointpillars} & L & 1.243   &  3.379 & 1.856  & 5.000  & 3.862& 5.000  &  1.752 & 4.512 \\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L& 0.906   &  3.379  & 1.065  & 3.807  & 2.478    & 4.161  & 1.444  &3.770  \\
BEVFusion \cite{liang2022bevfusion}& C+L &  1.054  & 3.035& 0.975  & 3.488  &  1.553   & 3.875  & 1.188  & 3.578 \\
BEVFusion \cite{liu2022bevfusion}& C+L&   1.071 &  3.504  & 1.022  & 3.745  & \textbf{1.447}    & 4.436  & 1.176  & 3.887 \\
SuperFusion (ours) & C+L&  \textbf{0.834}  &  \textbf{2.992}  &  \textbf{0.851} &  \textbf{2.988} & 1.543&  \textbf{3.824} & \textbf{1.066}  & \textbf{3.256} \\
\hline
\end{tabular}
% }
\normalsize
\end{table*}







% \begin{table*}[!tb]	
% \centering
% \addtolength{\tabcolsep}{0.5pt}
% \renewcommand\arraystretch{1}
% \setlength{\tabcolsep}{5pt}
% \caption{Chamfer distance (m) of semantic map segmentation on self-recorded dataset. CD: lower is better. }
% \label{tab:cd_haomo}
% \footnotesize
% % \scalebox{0.88}{
% \begin{tabular}{c|c|cc|cc|cc|cc}
% \hline
% \multirow{2.5}{*}{\textbf{Method}} &
% \multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{2}{c}{\textbf{{\scriptsize Average CD}}} \\

% & & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

% \hline 
% VPN \cite{Pan_2020} & C & 0.282  &  1.022 & 0.314 &  1.027&  0.456  & 0.904 & 0.341 & 0.996\\
% LSS \cite{philion2020lift} & C & 0.254  & 1.572  & \textbf{0.260} & 1.671 &  0.470  & 1.572 &0.324 & 1.610\\
% \hline
% PointPillars \cite{lang2019pointpillars} & L & 0.479   & 2.029  & 0.548  & 1.753 &  0.750  & 1.600 & 0.575& 1.850\\
% \hline 
% HDMapNet \cite{li2021hdmapnet}& C+L & 0.277  & 1.274  & 0.280 & 0.968 &  0.458  & \textbf{0.796} & 0.315 & 1.052\\
% BEVFusion \cite{liang2022bevfusion}& C+L & 0.296 & 1.250  & 0.337 & 1.479 & 0.588   &1.726  &0.403 & 1.464\\
% BEVFusion \cite{liu2022bevfusion}& C+L & 0.311   &2.173   & 0.288 & 2.135 &  0.516  & 2.394 &0.368 & 2.222\\
% SuperFusion (ours) & C+L & \textbf{0.235}  & \textbf{0.903}  & 0.280  & \textbf{0.858}   & \textbf{0.408}  & 0.932  &\textbf{0.302} & \textbf{0.894}\\
% \hline
% \end{tabular}
% % }
% \normalsize
% \end{table*}

==> tabs/ablation_turn.tex <==

\begin{table*}[!tb]	
\centering
\addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{3pt}
\caption{IoU scores (\%) of HD map generation in turning scenes on nuScenes dataset. We compare the results of HDMapNet and ours and show our performance improvement. Bold numbers are the best performance, and red numbers indicate larger improvements. }
\label{tab:ablation_turn}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|ccc|ccc|ccc|ccc}
\hline
\multirow{2.5}{*}{\textbf{}} &
\multirow{2.5}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{3}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{3}{c}{\textbf{{\scriptsize Average IoU}}} \\

& & {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Ped} } & {\textbf{Boundary} }\\

\hline 
\parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{original}}} & HDMapNet \cite{li2021hdmapnet} &  44.3 & 28.9 &55.4  &26.9  &10.4  &31.0  &18.1  &5.3 & 18.3 & 30.5& 16.6 &35.7\\
& SuperFusion (ours) & \textbf{47.9}  & \textbf{37.4} & \textbf{58.4} & \textbf{35.6} & \textbf{22.8} & \textbf{39.4} & \textbf{29.2} & \textbf{12.2}&  \textbf{28.1}&\textbf{38.0} & \textbf{26.2} &\textbf{42.7}\\
& Improvement  & +3.6  & +8.5 & +3.0 & +8.7 & +12.4 & +8.4 & +11.1 & +6.9 & +9.8 & +7.5 & +9.6 & +7.0\\
\hline
\parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{only turns}}} & HDMapNet \cite{li2021hdmapnet}& 42.8 & 27.8 &53.9  &24.6  &10.2  &27.6  & 17.1  & 4.3 & 16.0 & 29.2 &  14.4 & 32.7\\
& SuperFusion (ours) & \textbf{46.5}  & \textbf{37.0} & \textbf{57.6} & \textbf{33.5} & \textbf{22.7} & \textbf{38.5} & \textbf{28.4} & \textbf{11.9}&  \textbf{26.4}&\textbf{36.8} & \textbf{24.5} &\textbf{40.9}\\
& Improvement  & \red{+3.7}  & \red{+9.2} & \red{+3.7} & \red{+8.9} & \red{+12.5} & \red{+10.9} & \red{+11.3} & \red{+7.6} & \red{+10.4} & \red{+7.6} & \red{+10.1} & \red{+8.2}\\
\hline
\end{tabular}
% }
\normalsize
\end{table*}

==> tabs/segmentation_haomo.tex <==
% \begin{table}[!tb]	
% \centering
% \addtolength{\tabcolsep}{0.5pt}
% \caption{IoU scores (\%) of semantic map segmentation on HAOMO. IOU: higher is better.  }
% \label{tab:segmentation}
% \footnotesize
% \scalebox{0.88}{
% \begin{tabular}{c|c|cc}
% \hline
% \multirow{2.5}{*}{\textbf{Method}} &
% \multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c}{\textbf{Average}} \\

% & & {\textbf{Divider} } & {\textbf{Boundary} } \\

% \hline 
% VPN \cite{Pan_2020} & C & 42.9 & 17.9   \\
% LSS \cite{philion2020lift} & C & 49.2  & 20.4 \\
% \hline
% PointPillars \cite{lang2019pointpillars} & L & 36.8 &  15.5  \\
% \hline 
% HDMapNet \cite{li2021hdmapnet}& C+L &  46.6 & 18.8  \\
% BEVFusion \cite{liang2022bevfusion}& C+L &  48.1 & 21.9  \\
% BEVFusion \cite{liu2022bevfusion}& C+L &  49.0 & 18.8 \\
% SuperFusion (ours) & C+L & \textbf{51.2}  & \textbf{24.3}\\
% \hline
% \end{tabular}
% }
% \normalsize
% \end{table}

\begin{table*}[!tb]	
\centering
% \addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{5pt}
\caption{IoU scores (\%) of semantic map segmentation on self-recorded dataset. IoU: higher is better.  }
\label{tab:segmentation_haomo}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{2}{c}{\textbf{{\scriptsize Average IoU}}} \\

& & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C &  49.6 & 21.6  & 46.3  & 18.4 & 33.1  & 13.6& 42.9  & 17.9  \\
LSS \cite{philion2020lift} & C & 52.3  & 22.1  & 52.2  & 21.5 & 43.5  & 17.4   &  49.2 & 20.4  \\
\hline
PointPillars \cite{lang2019pointpillars} & L &  46.7 & 20.1  & 39.4  & 16.0 & 25.2  & 8.8   & 36.8  & 15.5  \\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L &  54.6 & 22.5  & 50.8  & 19.5 &  35.0 & 14.0&  46.6 & 18.8  \\
BEVFusion \cite{liang2022bevfusion}& C+L & 53.1  & 26.4  & 50.1  & 21.9 & 41.7  & 17.2   & 48.1  & 21.9  \\
BEVFusion \cite{liu2022bevfusion}& C+L &  51.9 & 21.4  & 51.7  & 20.0 & 43.6  & 15.3   & 49.0  & 18.8  \\
SuperFusion (ours) & C+L & \textbf{59.9}  & \textbf{28.4} & \textbf{55.2} & \textbf{25.2} & \textbf{44.2} & \textbf{20.4} & \textbf{53.0}  & \textbf{24.7}\\
\hline
\end{tabular}
% }
\normalsize
\end{table*}

==> tabs/supp_haomo.tex <==
\begin{table*}[!tb]	
\centering
% \addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{5pt}
\caption{IoU scores (\%) of semantic map segmentation on HAOMO. IOU: higher is better.  }
\label{tab:segmentation_haomo}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{2}{c}{\textbf{{\scriptsize Average}}} \\

& & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C &  49.6 & 21.6  & 46.3  & 18.4 & 33.1  & 13.6& 42.9  & 17.9  \\
LSS \cite{philion2020lift} & C & 52.3  & 22.1  & 52.2  & 21.5 & 43.5  & 17.4   &  49.2 & 20.4  \\
\hline
PointPillars \cite{lang2019pointpillars} & L &  46.7 & 20.1  & 39.4  & 16.0 & 25.2  & 8.8   & 36.8  & 15.5  \\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L &  54.6 & 22.5  & 50.8  & 19.5 &  35.0 & 14.0&  46.6 & 18.8  \\
BEVFusion \cite{liang2022bevfusion}& C+L & 53.1  & 26.4  & 50.1  & 21.9 & 41.7  & 17.2   & 48.1  & 21.9  \\
BEVFusion \cite{liu2022bevfusion}& C+L &  51.9 & 21.4  & 51.7  & 20.0 & 43.6  & 15.3   & 49.0  & 18.8  \\
SuperFusion (ours) & C+L & \textbf{59.9}  & \textbf{28.4} & \textbf{55.2} & \textbf{25.2} & \textbf{44.2} & \textbf{20.4} & \textbf{53.0}  & \textbf{24.7}\\
\hline
\end{tabular}
% }
\normalsize
\end{table*}



\begin{table*}[!tb]	
\centering
\addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{5pt}
\caption{Chamfer distance (m) of semantic map segmentation on HAOMO. CD: lower is better. }
\label{tab:cd_haomo}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}} & \multicolumn{2}{c}{\textbf{{\scriptsize Average}}} \\

& & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C & 0.282  &  1.022 & 0.314 &  1.027&  0.456  & 0.904 & 0.341 & 0.996\\
LSS \cite{philion2020lift} & C & 0.254  & 1.572  & \textbf{0.260} & 1.671 &  0.470  & 1.572 &0.324 & 1.610\\
\hline
PointPillars \cite{lang2019pointpillars} & L & 0.479   & 2.029  & 0.548  & 1.753 &  0.750  & 1.600 & 0.575& 1.850\\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L & 0.277  & 1.274  & 0.280 & 0.968 &  0.458  & \textbf{0.796} & 0.315 & 1.052\\
BEVFusion \cite{liang2022bevfusion}& C+L & 0.296 & 1.250  & 0.337 & 1.479 & 0.588   &1.726  &0.403 & 1.464\\
BEVFusion \cite{liu2022bevfusion}& C+L & 0.311   &2.173   & 0.288 & 2.135 &  0.516  & 2.394 &0.368 & 2.222\\
SuperFusion (ours) & C+L & \textbf{0.235}  & \textbf{0.903}  & 0.280  & \textbf{0.858}   & \textbf{0.408}  & 0.932  &\textbf{0.302} & \textbf{0.894}\\
\hline
\end{tabular}
% }
\normalsize
\end{table*}


\begin{table*}[!tb]	
\centering
\addtolength{\tabcolsep}{0.5pt}
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{5pt}
\caption{Instance detection results on HAOMO. The predefined threshold of Chamfer distance is 1.0 m and threshold of IoU is 0.1 (\eg a prediction is considered a true positive if the Chamfer distance between label and prediction is lower than that threshold). AP: higher is better.}
\label{tab:ap_haomo}
\footnotesize
% \scalebox{0.88}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\multirow{2.5}{*}{\textbf{Method}} &
\multirow{2.5}{*}{\textbf{Modality}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 0-30 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 30-60 m}}} & \multicolumn{2}{c|}{\textbf{{\scriptsize 60-90 m}}}& \multicolumn{2}{c}{\textbf{{\scriptsize Average}}}\\

& & {\textbf{Divider} }& {\textbf{Boundary} } & {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }& {\textbf{Divider} } & {\textbf{Boundary} }\\

\hline 
VPN \cite{Pan_2020} & C & 40.9  &28.9   &36.2  & 27.1 & 21.9   & 20.0  & 33.0 & 25.4\\
LSS \cite{philion2020lift} & C & 42.8  & 28.9  & 42.7 & 27.7 & 35.8   & 22.9 & 40.4 &26.5 \\
\hline
PointPillars \cite{lang2019pointpillars} & L & 30.7   & 29.0  & 28.0  & 27.6 &  19.7  & 17.2 &  26.1& 24.6\\
\hline 
HDMapNet \cite{li2021hdmapnet}& C+L & 44.9  & 29.2  & 43.0 & 28.1 &  27.1  & 19.9 & 38.3 & 25.7\\
BEVFusion \cite{liang2022bevfusion}& C+L & 42.1 & 34.2  & 40.4 & 31.9 & 33.9   &25.2  & 38.8 & 30.5\\
BEVFusion \cite{liu2022bevfusion}& C+L & 43.0   & 28.8  &42.6  & 27.5 & \textbf{35.9}   &21.4  &40.5  &25.9 \\
SuperFusion (ours) & C+L & \textbf{47.5}  & \textbf{38.0} & \textbf{44.3} & \textbf{36.8}  &35.3  & \textbf{30.0}  & \textbf{42.4} & \textbf{35.0} \\
\hline
\end{tabular}
% }
\normalsize
\end{table*}


